Bandit learning in concave $N$-person games

This paper examines the long-run behavior of learning with bandit feedback in non-cooperative concave games. The bandit framework accounts for extremely low-information environments where the agents may not even know they are playing a game; as such, the agents' most sensible choice in this setting would be to employ a no-regret learning algorithm. In general, this does not mean that the players' behavior stabilizes in the long run: no-regret learning may lead to cycles, even with perfect gradient information. However, if a standard monotonicity condition is satisfied, our analysis shows that no-regret learning based on mirror descent with bandit feedback converges to Nash equilibrium with probability $1$. We also derive an upper bound for the convergence rate of the process that nearly matches the best attainable rate for single-agent bandit stochastic optimization.

==> Algorithms/DA.tex <==
%----------------------------------------------------------------------
%%% DA ALGORITHM
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\begin{algorithmic}[1]
\Require
%	$\strong$-strongly convex regularizer $\hreg\from\feas\to\R$,
	step-size $\step_{\run}>0$
\State
	initialize score vector $\score\in\dspace$
	\Comment{initialization}%
\Repeat\;
	at each stage $\run=\running$
	\State
		play $\act\leftarrow\mirror(\score)$
		\Comment{choose action}%
	\State
		get $\est\payv$
		\Comment{oracle feedback}%
	\State
		update $\score \leftarrow \score + \step_{\run} \est\payv$
		\Comment{update scores}%
\Until{end}
\end{algorithmic}

==> Algorithms/MD.tex <==
%----------------------------------------------------------------------
%%% MP ALGORITHM
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\begin{algorithmic}[1]
\Require
	$\strong$-strongly convex regularizer $\hreg\from\feas\to\R$,
	step-size sequence $\step_{\run}>0$
\State
	choose $\act\in\dom\subd\hreg$
	\Comment{initialization}%
\For{$\run=\running$}
	\State
		get $\est\payv$
		\Comment{gradient estimate}%
	\State
		set $\act \leftarrow \prox_{\act}(\step_{\run}\est\payv)$
		\Comment{update state variable}%
\EndFor
\end{algorithmic}

==> App-Preamble.tex <==
%----------------------------------------------------------------------
%%% APP: PREAMBLE
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


For completeness, we briefly reproduce here some basic definitions concerning the most important elements of our paper.

First, given a $\strong$-strongly convex regularizer $\hreg\from\feas\to\R$ (the player index $\play$ is suppressed for simplicity), the associated Bregman divergence is defined as
\begin{equation}
\label{supp-eq:Bregman}
\breg(\base,\state)
	= \hreg(\base) - \hreg(\state) - \braket{\nabla\hreg(\state)}{\base - \state}
\end{equation}
with $\nabla\hreg(\state)$ denoting a continuous selection of $\subd\hreg(\state)$.
The induced prox-mapping is then given by
\begin{flalign}
\label{supp-eq:prox}
\prox_{\state}(\dstate)
	&= \argmin_{\alt\state\in\feas} \{ \braket{\dstate}{\state - \alt\state} + \breg(\alt\state,\state) \}
	\notag\\
	&= \argmax_{\alt\state\in\feas} \{ \braket{\dstate + \nabla\hreg(\state)}{\alt\state} - \hreg(\alt\state) \}
\end{flalign}
and is defined for all $\state\in\dom\subd\hreg$, $\dstate\in\dspace$ (recall here that $\dspace \equiv \dual\vecspace$ denotes the dual of the ambient vector space $\vecspace$ in which the game's action space $\feas$ is embedded).%
\footnote{We also recall here that $\dspace$ comes naturally equipped with the dual norm $\dnorm{\dstate} = \max\setdef{\abs{\braket{\dstate}{\state}}}{\norm{\state} \leq 1}$.}

With all this at hand, the multi-agent \acl{MD} algorithm with bandit feedback is defined as follows:
\begin{equation}
\label{supp-eq:MD-0}
\tag{MD-b}
\begin{aligned}
\est\act_{\run}
	&= \act_{\run} + \mix_{\run} \pertvar_{\run},
	\\
\act_{\run+1}
	&= \prox_{\act_{\run}}(\step_{\run}\est\payv_{\run}).
\end{aligned}
\end{equation}
where the perturbation $\pertvar_{\run}$ and the estimate $\est\payv_{\run}$ are given respectively by
\begin{equation}
\pertvar_{\play,\run}
	= \unitvar_{\play,\run} - \radius_{\play}^{-1} \parens{\act_{\play,\run} - \base_{\play}}
%	\quad
%	\text{and}
	\qquad
\est\payv_{\play,\run}
	= (\vdim_{\play}/\mix_{\run}) \pay_{\play}(\est\act_{\run}) \, \unitvar_{\play,\run}.
\end{equation}
In the above, the query directions $\unitvar_{\play,\run}$ are drawn independently and uniformly across players at each stage $\run$ from the corresponding unit sphere;
finally,
$\ball_{\radius_{\play}}(\base_{\play})$ denotes a ball that is entirely contained in $\feas_{\play}$.
For a schematic representation, see also \cref{fig:MD-0}.
